SnAG: Scalable and Accurate Video Grounding

Temporal grounding of text descriptions in videos is a central problem in vision-language learning and video understanding. Existing methods often prioritize accuracy over scalability -- they have been optimized for grounding only a few text queries within short videos, and fail to scale up to long videos with hundreds of queries. In this paper, we study the effect of cross-modal fusion on the scalability of video grounding models. Our analysis establishes late fusion as a more cost-effective fusion scheme for long-form videos with many text queries. Moreover, it leads us to a novel, video-centric sampling scheme for efficient training. Based on these findings, we present SnAG, a simple baseline for scalable and accurate video grounding. Without bells and whistles, SnAG is 43% more accurate and 1.5x faster than CONE, a state of the art for long-form video grounding on the challenging MAD dataset, while achieving highly competitive results on short videos.

==> tables/dataset_stats.tex <==
\resizebox{\linewidth}{17mm}{
\begin{tabular}{lcccccc}
\toprule[1.5pt]
  & \#~Video & \#~Query & \#~Query & $\bar{L}_{video}$ &$\bar{L}_{query}$ & $\bar{L}_{moment}$ \\
\multirow{-2}{*}{Dataset} & (train~/~test) &(train~/~test) & /~Video & (min) & (word) & (sec) \\ \midrule[0.5pt]
MAD~\cite{soldan2022mad} & 488~/~112 & 28.0K~/~72.0K & 630.5 & 110.77 & 12.7 & 4.1 \\
Ego4D-NLQ~\cite{grauman2022ego4d} & 998~/~328 & 11.3K~/~3.9K & 11.6 & 8.25 & 8.6 & 3.9 \\
TACoS~\cite{regneri2013tacos} & 75~/~25 & 9.8K~/~4.0K & 143.5 & 4.78 & 10.5& 27.9 \\
\specialrule{0em}{2pt}{2pt}
Charades-STA~\cite{sigurdsson2016charades} & 5.3K~/~1.3K & 12.4K~/~3.7K & 1.6 & 0.50 &7.2 & 8.1 \\
ANet-Captions~\cite{gao2021ranet} & 10.0K~/~4.9K & 37.3K~/~17.0K & 3.6 & 1.96 &14.8 & 37.3   \\
\bottomrule[1.5pt]
\end{tabular}
}

==> tables/dataset_stats_table_and_figure.tex <==
\begin{figure*}
    
    \begin{minipage}{0.3\linewidth}
    \includegraphics[width=\linewidth]{fig/datasets.pdf} %\vspace{-1.5em}
    \label{fig:data_split}
    \end{minipage}
    % \hspace{-0.5em}
    %\hfill
    \begin{minipage}{0.6\linewidth}
 \vspace{-2em}

\begin{tabular}{lccccc}
\toprule[1.5pt]
                          & \#~Video                                & \#~Query                                & \#~Query                        & $\bar{L}_{video}$ & $\bar{L}_{moment}$ \\
\multirow{-2}{*}{Dataset} & (train~/~test) &(train~/~test) & /~Video & (min) & (sec)  \\ \midrule[0.5pt]
MAD~\cite{soldan2022mad}                       & 488~/~112                              & 28.0K~/~72.0K                          & 630.5                          & 110.77 & 4.1     \\
Ego4D-NLQ~\cite{grauman2022ego4d}                 & 998~/~328                              & 11.3K~/~3.9K                           & 11.6                           & 8.25   & 3.9     \\
TACoS~\cite{regneri2013tacos}                     & 75~/~25                                & 9.8K~/~4.0K                            & 143.5                          & 4.78   & 27.9    \\
\specialrule{0em}{2pt}{2pt}
Charades-STA~\cite{sigurdsson2016charades}              & 5.3K~/~1.3K                            & 12.4K~/~3.7K                           & 1.6                            & 0.50   & 8.1     \\
ANet-Captions~\cite{gao2021ranet}             & 10.0K~/~4.9K                           & 37.3K~/~17.0K                          & 3.6                            & 1.96   & 37.3   \\
\bottomrule[1.5pt]
\end{tabular}


\label{table:dataset_stats}
\end{minipage}



    \caption{\textbf{Comparison of video-language grounding datasets.} The circle size measures the number of queries per video}
    \label{fig:datasets}
\end{figure*}

==> tables/train_scale.tex <==
\begin{table}[]
\begin{tabular}{lllllll}
\toprule[1.5pt]
              & 256  & 512   & 1024  & 2048  & 4096  & 8192  \\
\hline
R@1, tIoU=0.5 & 3.31 & 4.06  & 4.73  & 5.24  & 5.55  & 5.73  \\
R@5, tIoU=0.5 & 9.04 & 10.64 & 11.94 & 13.02 & 13.75 & 14.06 \\
\bottomrule[1.5pt]
\end{tabular}
\end{table}
